Language Evolution for Evading Social Media Regulation via LLM-based Multi-agent Simulation

Social media platforms such as Twitter, Reddit, and Sina Weibo play a crucial role in global communication but often encounter strict regulations in geopolitically sensitive regions. This situation has prompted users to ingeniously modify their way of communicating, frequently resorting to coded language in these regulated social media environments. This shift in communication is not merely a strategy to counteract regulation, but a vivid manifestation of language evolution, demonstrating how language naturally evolves under societal and technological pressures. Studying the evolution of language in regulated social media contexts is of significant importance for ensuring freedom of speech, optimizing content moderation, and advancing linguistic research. This paper proposes a multi-agent simulation framework using Large Language Models (LLMs) to explore the evolution of user language in regulated social media environments. The framework employs LLM-driven agents: supervisory agent who enforce dialogue supervision and participant agents who evolve their language strategies while engaging in conversation, simulating the evolution of communication styles under strict regulations aimed at evading social media regulation. The study evaluates the framework's effectiveness through a range of scenarios from abstract scenarios to real-world situations. Key findings indicate that LLMs are capable of simulating nuanced language dynamics and interactions in constrained settings, showing improvement in both evading supervision and information accuracy as evolution progresses. Furthermore, it was found that LLM agents adopt different strategies for different scenarios.

==> Evaluation.tex <==
\section{Evaluation}
\label{sec: evaluation}
%为了验证我们系统的有效性和对语言演化的影响，我们设计了三个不同场景的实验。这些实验旨在模拟不同的监管环境下参与者的对话行为，并观察其策略如何演化以适应监管者的规则。
%我们的研究将围绕以下几个问题展开：
% RQ1: LLM驱动的agent能否有效地进行语言演化? 以规避监管的同时传播内容。
% RQ2: 语言是怎么演化的，演化策略和演化倾向（成功和失败的策略分别是什么样的）
% (optional)RQ3: 针对不同程度的监管力度agent下语言演化策略是否发生变化。
% (optional)RQ4:不同的LLM的语言演化过程有着怎样的区别？

\subsection{Experiment Setting}
在这项研究中，我们使用以大语言模型（LLM）为基础的多代理模拟系统探索了各种监管环境中代理的适应性和战略演变。我们的研究涵盖了各种场景，从理论和抽象测试到反映复杂现实情况的模拟。主要目的是评估LLM在不同语言环境中的适应性及其在实际监管框架中的潜在应用。从简单的理论设置开始，逐渐转变为复杂的现实生活，以渐进的方式进行实验。这种方法旨在在不同的设置中对LLM的功能提供全面的了解。

\subsubsection{Case 1: 猜数字情景 (2人理论能力测试)}
我们的第一个场景考虑了一个较为单一且抽象的猜数字场景。在此场景中，每一位参与者都会被赋予一个1-100正整数范围内的值，参与者需要通过数论对话在不直接提及数字的前提下将自身的值传达给别的参与者，同时也需要从对话中获取信息以推理出对方的值。而监管者会遵循“禁止对话中一切与数字相关的内容”这一Guideline来对对话内容进行监管。“猜数字”场景专门设计用于观察和分析参与者在一个理论化且较为抽象的情景下的语言适应性和策略演化，与更为复杂的基于现实中真实事件的场景相比，此场景提供了更为简明且可控的实验环境。我们将专注于分析随演化次数增加，参与者间对话被监管者发现的回合数变化，以及这与猜数字精度之间的关系。总的来说，这个简化且理论化的场景展现了LLM在监管下语言演化方面最接近于理论性能的能力，包括且不限于语言编码，解码以及推理能力。

\subsubsection{Case 2: 非法宠物交易}
在这个场景中，我们模拟了通过社交媒体进行非法动物交易的情境。参与者分别扮演买家和卖家，买家需要向卖家传达购买诉求，会在鹦鹉，蜥蜴和猫中随机选定一个。而卖家则需要根据买家购买的宠物种类不同，提供不同的交易信息。交易信息具体为三项，时间地点和人物。监管者的任务是阻止任何药品交易对话。我们将通过采访对双方理解的信息进行交叉验证，评估信息传播的成功率。这个实验的关键在于观察参与者在较大的信息粒度上的语言适应性和演化，以及监管者如何准确识别相关对话。我们将分析对话内容的演化曲线、编码方式和信息传递的准确性，以衡量参与者的适应性和监管者的有效性。

\subsubsection{Case 3: 核废水情景 (多人类现实情景测试，观点传递)}
这个场景贴近现实中的复杂事件，涉及日本政府处理福岛第一核电站事故后积累的放射性废水排放问题。此计划虽获得国际原子能机构支持，但也面临来自中国、韩国等国家和国际组织的环保担忧和反对，引发了中韩日社交网络上的激烈讨论。在此情景下，我们模拟了一个多人在监管环境下进行论坛发帖讨论的场景，围绕福岛核废水处理的争议性话题。参与者需要表达各自的立场和论据，而监管者的任务是确保讨论不涉及环境污染和日本政府的敏感话题。实验结束后，我们将对参与者进行采访，了解他们对事件的看法。此场景不仅考察语言规避能力和演化次数，还着重于LLM对于具体真实事件论据的编码方式演变以及对编码后信息的解码能力。

\subsection{Experiment Result}


\subsection{Discussions}



==> Method.tex <==
\section{System Design}
\label{sec: method}
%\jialong{结构有点乱，建议分成overview，superviosr, participant三个subsection来写}
%原文在下面的Method.tex里
This research develops a sophisticated multi-agent simulation framework using LLMs, aimed at examining the adaptive evolution of language strategies to circumvent social media regulation. The framework comprises two core roles: the Supervisor, tasked with enforcing established guidelines, and the Participant, whose goal is to convey specific, human-defined information discreetly. Participants must dynamically refine their communication approaches, drawing from past dialogues, to transmit information effectively while remaining undetected. This section provides a comprehensive system overview and delves into the technical aspects of both Participants and the Supervisor.

\jialong{感觉还是ABC三方的player都画出来，然后反思和规划画成agent内部的交互流程，然后不同agent之间的交互是外部交互流程}
\begin{figure*}[htbp]
	\centering
	\includegraphics[width=0.8\linewidth]{paper/figures/flow.png}
	\caption{Unfinished}
        \label{fig:overview}
\end{figure*}

\subsection{Overview}
\label{subsec: overall_system_architecture}
In this section, we delineate the comprehensive structure of our system, illustrated in Figure\ref{fig:overview}. Central to our framework are two types of entities: multiple dialogue participant agents and a singular abstract supervisor agent, all powered by LLMs. The system begins with the initialization of each agent, incorporating their designated roles, background information, and primary tasks. Subsequently, participant agents engage in dialogues. After each dialogue session, the supervisor agent assesses the exchange against established guidelines. When deviations from these guidelines are detected, the supervisor intercedes by halting the dialogue and specifying the segments of text that contravened the guidelines, along with the rationale for such a determination. These interactions and the supervisor's guideline-related feedback are systematically archived in the "Dialogue History" and "Violation Log," respectively.

Before commencing a new round of dialogue, participant agents utilize a reflection module to strategize how to navigate around the guidelines, drawing insights from the "Violation Log." This leads to the creation of "Regulations" that inform the participants' dialogue strategies, aiming to circumvent supervisor detection. The dialogue continues for a series of turns until it reaches an interview phase without supervisor intervention. In this phase, agents are interrogated about their interpretations of their counterparts' conveyed messages. After the interview, a summarization module is activated, allowing agents to cross-examine the gathered information from the interviews. This process helps in identifying key learnings from their communication approaches, both where they succeeded and where they failed. These learnings, referred to as "Guidance," are then applied to refine the accuracy and effectiveness of future dialogues in terms of message delivery.

\subsection{Participant}
In this framework, the Participant agent includes multiple modules aimed at ensuring accurate information delivery while evading supervision. These modules include a Memory module, Dialogue module, Reflection module, and Summary module. To enhance system flexibility and reduce redundant information, we subdivided the Prompts of each module into six main elements: “Background Information,” “Dialogue History,” “Violation Log,” “Regulations,” “Guidance,” and “Instructions.” “Background Information” provides necessary information and objectives related to the experimental scenario. “Dialogue History” and “Violation Log,” managed by the Memory module, record the past dialogues among Participants and the records detected by the Supervisor, respectively. Expressing regulated topics effectively while evading supervision poses a significant challenge to the LLM’s linguistic capabilities. Therefore, we introduced “Regulations” and “Guidance,” two key elements generated by the Reflection and Summary modules, to guide the agent in avoiding supervision and effectively conveying information. “Instructions” contain the core directives of the current Prompt. We will now introduce each module in detail.

\subsubsection{Dialogue Module}
This module is responsible for generating dialogue content based on short-term conversation records. It extracts historical dialogue information from the Memory module and inputs it into the LLM to understand and construct sentences, ensuring the communication content can evade supervision and effectively convey information. In the Prompt of the Dialogue module, “Background Information” provides the required background information, while “Regulations” and “Guidance” guide the necessary precautions for achieving the objective. “Instructions” offer the LLM's specific execution instructions.

\subsubsection{Memory Module}
The Memory module stores all dialogue history and records detected by the Supervisor, crucial for Participants to understand the supervision pattern and improve future dialogue strategies. Specifically, the Memory module is divided into three parts: Task Background, Dialogue History, and Violation Record. Task Background includes role setting, experimental background knowledge, and objectives. “Dialogue History” and “Violation Log” save the dialogue records and the records detected by the Supervisor in the past, respectively. “Dialogue History,” as temporary memory, only contains the current round of dialogue. “Violation Log,” as long-term memory, records violation information in each evolutionary round. When dialogue is detected by the Supervisor, relevant feedback is added to the “Violation Log,” triggering a new round of evolution. Given that the number of tokens LLM can process is limited and longer prompts may cause issues such as information forgetting in LLM, when the text volume of “Dialogue History” and “Violation Log” exceeds a certain threshold, memory compression will be performed, prioritizing older records. Memory compression is also executed by the LLM.

\subsubsection{Reflection Module}
The Reflection module is activated at the start of each evolutionary round. It infers the Supervisor's guiding principles by analyzing detected records and generates corresponding strategies (“Regulations”) to better adapt to the supervision environment. To reduce redundancy in the Prompt, the external information input of the Reflection module is limited to the “Violation Log,” allowing the LLM to accurately analyze and summarize past failure records. The LLM must possess a high degree of reasoning ability to infer the principles driving the Supervisor from superficial failure records and formulate appropriate strategies (“Regulations”). We have adopted the effective and cost-efficient COT (Chain of Thought) method as the guiding idea in the Reflection module, directing the LLM to analyze the principles and generate strategies combined with the main task (Figure?).

\subsubsection{Summary Module}
The Summary module comes into play when the dialogue fails to effectively convey information. It reviews and analyzes the dialogue content, proposing improvements (“Guidance”) to help Participants more effectively convey their viewpoints. The Summary module is similar to the Reflection module but focuses more on completing information transmission rather than just evading supervision. Therefore, the additional information input of the Summary module includes only “Dialogue History.”

\subsection{Supervisor}
The role of the Supervisor in this study is a key link in the dialogue framework. Its duty is to supervise the Participants' dialogue and ensure that the content complies with established guiding principles. The Supervisor's agent in this study is also driven by the LLM. In each experiment, researchers provide the experimental background and guidelines for the Supervisor as shown in Figure?. Unlike the Participant, the Supervisor's architecture and Prompt design are relatively simple. "Background Information" provides the necessary background information for the task. "Dialogue History" represents the dialogue between agents in the current round. The Instruction specifies the guidelines the Supervisor agent must follow to complete the dialogue inspection.

To explore the impact of different supervision pressures on the Participants' evolutionary strategies in experiments, the Supervisor needs the ability to adjust the supervision pressure. However, both in reality and in simulated environments, supervision pressure is often a concept difficult to quantify. Therefore, we use a mixed Prompt method of concept + example to achieve three different levels of supervision pressure (Figure?), which are: direct mention, indirect mention, and abstract involvement. (For example, describing grapes would be direct: grape, indirect: purple fruit the size of a coin. Abstract: strings of sour-sweet purple gems.)

Lastly, it's worth noting that in this framework, supervision pressure depends not only on the impact of prompt settings but also on the influence of the LLM's semantic understanding and reasoning abilities. Simply put, under the same prompt premise, an LLM with stronger semantic understanding and reasoning capabilities will typically exert greater supervision pressure than an LLM with weaker abilities. Therefore, we can also use different LLMs to achieve different supervision pressures under the same prompt.




\section{System Design}
\label{sec: method}
%本研究构建了一个抽象的社交网络监管环境下的对话框架，涵盖了监管者（Supervisor）和参与者（Participant）两个关键角色。参与者的主要任务是传递人为定义的特定信息的同时不被监管到，而监管者则负责确保对话内容符合既定规则。在这种情境下，参与者必须基于自身以往的经验，不断演化和更新自己的沟通策略，以有效传递信息同时避免被监管者发现。在this section中，我们先会介绍整个系统的overview，然后会分别介绍参与者与监管者各自具体的技术要点。
\subsection{参与者}
%在本框架中，参与者代理包含多个模块，旨在确保信息的准确传递同时规避监管。这些模块包括记忆模块、对话模块、反思模块和规划模块。为实现系统的灵活性并减少冗余信息，我们将各模块的Prompt进行细分，共分为六个主要元素：“Background Information”、“Dialogue History”、“Violation Log”、“Regulations”、“Guidance”,"Plan"和“Instructions”。其中，“Background Information”提供了实验场景的相关必要信息及目标。“Dialogue History”和“Violation Log”由记忆模块管理，分别记录着过去参与者间的对话和被监管者发现的记录。在受监环境下，有效地表达监管话题同时规避监管，对LLM的语言能力是一个极大的挑战。因此，我们引入了“Regulations”,“Guidance”和“Plan”三个关键元素，分别由反思模块和规划模块生成，以指导代理在避免被监管和有效传递信息方面的行动。“Instructions”则包含了本次Prompt的核心指示。接下来，我们将对每个模块进行详细介绍。

\subsubsection{对话模块}
%该模块负责根据短期对话记录生成对话内容。从记忆模块中提取历史对话信息，并输入给LLM，以理解和构造语句，确保沟通内容既能规避监管，又能有效传递信息。在对话模块的Prompt中，“Background Information”提供了所需的背景信息，“Plan”指导了为了达成目标的所需的规划。“Instructions”则给出了LLM当前的具体执行指令。
\subsubsection{记忆模块}
%记忆模块存储所有对话历史和被监管者检测到的记录，对于参与者理解监管模式和改进未来对话策略至关重要。具体而言，记忆模块分为三部分：任务背景、对话历史和违规记录。任务背景包括角色设定、实验背景知识及目标。“Dialogue History”和“Violation Log”分别保存了对话记录和过去被Supervisor检测到的记录。“Dialogue History”作为临时记忆，仅包含当前回合的对话。“Violation Log”作为长期记忆，记录在每轮演化中的违规信息。当对话被监管者检测到，相关反馈会被加入“Violation Log”，从而触发新一轮的演化过程。鉴于LLM处理的token数量有限，并且越长的prompt可能会引发LLM的信息遗忘等问题，因此当“Dialogue History”和“Violation Log”的文本量超过一定阈值时，将进行记忆压缩，优先处理较旧的记录。记忆压缩同样由LLM执行。

\subsubsection{反思模块}
%反思模块在每一轮对话演化的开始和结束时被激活，其核心目的是基于历史记录生成改进策略。在演化周期的初期，反思模块以“Violation Log”（违规日志）作为输入，分析过往的失败经验，并据此制定“Regulations”（规则），以期在未来的对话中有效规避监管。而在每个周期的末尾，反思模块再次启用，这时它将关注“Dialogue History”（对话历史），目的是回顾并评估对话内容，检查是否成功完成了主要任务中的信息表达。若发现信息表达不充分或未达到预期目标，则需提出相应的“Guidance”（指导），用于指导后续的对话，从而增强代理的信息传达效能。这样的设计使反思模块成为系统中关键的自我评估和策略调整机制，确保了对话系统在动态变化的监管环境中的连续进步和适应性。

%为了能够实现这些需求，LLM需具备高度的推理能力，不仅能从失败记录中推断出监管者的准则，还能从对话历史中提炼出沟通的不足，进而制定适当的策略和改进建议。为了提升LLM的推理能力，prompt的设计中我们采用了有效且成本低的COT方法作为反思与规划模块的指导思想，引导LLM进行准则分析并结合主要任务生成“Regulations”和“Guidance”。


\subsubsection{规划模块}
在监管环境下进行信息交流本身是一个充满挑战且矛盾的过程。其中，“Regulations”（规则）的部分聚焦于规避监管的策略，而“Guidance”（指导）则侧重于信息的有效表达。尽管这两个方面各自对对话管理至关重要，但在特定的监管环境中，它们可能会相互冲突，从而影响整体的语言表现和效率。因此，引入规划模块至关重要，其作用在于综合“Regulations”和“Guidance”的原则，形成一个具有实际指导性的“Plan”（计划），旨在为后续对话提供明确且有效的方向。这种将规避监管的规则和信息表达指导分别推理再结合的方法，不仅有助于在复杂的监管环境中平衡和优化语言演化的动机，提高对话系统的策略效率和适应性，同时也为研究者提供了一个清晰的框架，以更深入地理解和分析agent行为背后的动力。


\subsection{监管者}
%在本研究中，监管者的角色被设计为一个抽象的概念，主要用来模拟社交网络中的监管行为。这种设计反映了一个重要的观察：在社交网络中，内容的监管过程往往集中于对特定信息的直接判断，很少会受到广泛或长篇幅的上下文信息的影响。所以与具有更多复杂背景信息的参与者不同，监管者的功能和角色在这里被简化，以突出其在实际社交网络监管中的行为特征。监管者的任务主要聚焦于评估内容是否符合特定的标准或规则，这是一个相对直接且定义明确的过程。prompt中的内容仅包含了"Dialogue History"和"Instruction"。"Dialogue History"为该回合参与者agent之间的对话内容，Instruction则指定了监管者agent需要遵循的guideline以完成对对话的监察。

%为了在实验中探究不同的监察压力对于参与者的演化策略有着怎样的影响，监管者需要具备调整监察压力的可能性。然而无论现实中还是模拟环境中，监察压力往往是一个非常难以进行量化的概念。我们提出了一个混合架构的三阶段的压力设定方式，分别命名为：直接，间接以及抽象。在直接等级中，我们使用关键词搜索来判断是否违规，间接与抽象的等级我们使用LLM进行判断，通过概念+示例的混合prompt方式以实现不同的监管压力。（配图的例子的话，形容葡萄就是 直接：葡萄 间接：紫色硬币大小的果实。抽象：一串串酸甜的紫色宝石）

%最后，值得注意的是，在本框架中，监管压力不仅取决于prompt设置的影响，还取决于LLM的语义理解以及推理能力带来的影响。简单来说，相同的prompt的前提下，有着更强语义理解以及推理能力的LLM往往比语义理解以及推理能力更弱的LLM比会给出更大的监管压力。因此我们也可以将使用不同LLM以实现相同prompt下不同的监管压力。



\subsection{Overall flow}
在本节中，我们会介绍我们的系统的overview。图？展示了我们的系统的整体框架。系统主要由两种角色组成：复数的对话参与者agent与一个抽象的监管者agent。在整个系统中，无论参与者还是监管者，行动均由LLM所驱动。首先我们会初始化每个agent的基本信息，这包括角色设定，背景知识，主要任务等信息。之后，参与者agent之间会互相发起对话，在每一轮对话后，监管者会审查对话是否违反预先设定的规则。如果违反的话，监管者会强制中止本次对话，并给出违反的文本信息以及理由。在这个过程中，参与者agent之间的对话以及监管者给出的违反的文本信息等都会被被分别保存到“Dialogue History”和“Violation Log”之中。为了规避监管，在新的一次对话开始前，参与者agent会使用反思模块根据Violation Log中的失败记录生成对应避开监管的Regulations。Regulations对参与者agent生成的对话有着指导作用。如果在没有被监管者监管到的情况下对话持续一定回合后会结束对话进入采访环节。采访会对每个参与agent认为的对方想要表达的内容进行采集。采访后会再次进入反思模块以进行评估，反思模块会让agent交叉验证采访环节中采访到的内容，总结失败或者成功的经验作为Guidance来影响未来的对话以提升表达的准确率。为了更加直接有效的指导对话内容，规划模块会在每次Regulations或者Guidance被更新时启用以生成plan。
 
%本节旨在概述本研究所构建的对话框架在监管环境下的整体工作流程。这一流程反映了参与者与监管者之间的动态互动，以及他们如何在每轮对话中调整和演化自己的策略。
%模块初始化：首先，我们初始化所有关键模块，包括反思模块、对话模块、规划模块和记忆模块。同时，建立一个用于记录违规内容的日志（Violation Log）。
%角色设定：在每轮迭代中，我们设定参与者列表和监管者角色。这一步骤确保了每次对话都有新的动态和挑战。
%对话与监管：参与者通过对话模块生成对话内容，并提交给监管者进行内容合规性的审核。
%违规处理：如果监管者发现违规内容，该内容将被记录到违规日志中，并立即中断当前对话流程。
%记忆更新与分析：对话内容被存储到记忆模块中，供后续分析和策略调整之用。
%策略迭代：通过反思模块和规划模块，参与者基于以往的对话和违规记录来改进自己的沟通策略。
%持续演化：该流程持续重复，模拟参与者在监管环境下的对话策略和行为模式的持续演化。
%通过这种方式，我们的系统不仅能够深入探索社交网络监管环境下的沟通动态，还能提供实用的策略和反馈，以优化沟通效果并适应监管的变化。
\begin{algorithm}
\caption{Main flow}
\begin{algorithmic}[1]
\label{alg:1}
\State Initialize reflection, dialogue, summary, memory modules: $M_r$, $M_d$, $M_s$, $M_m$
\State Initialize violation log: $V\_log$

\While{true}
    State Initialize participants list $P$ with elements $p_1, p_2, \ldots, p_n$
    \State Initialize supervisor $S$
    \If{length($V\_log$) $\geq 2$}
        \State Apply reflection module $M_r$ to each participant in $P$
    \EndIf
    \For{a fixed number of iterations}
        \State Initialize dialogue list for this iteration: $D\_list$
        \ForAll{participants in $P$}
            \State Call the dialogue module $M_d$ for the current participant
            \State Add output from $M_d$ to $D\_list$
        \EndFor
        \State Submit dialogue records in $D\_list$ to $S$ for violation check
        \If{violation found}
            \State Add violation to $V\_log$
            \State \textbf{break}
        \EndIf
        \State Add $D\_list$ to memory module $M_m$
    \EndFor
    \State Interview each participant in $P$
    \State Execute summary module$M_s$ for each participant in $P$
\EndWhile
\end{algorithmic}
\end{algorithm}

